Unveiling User Behavior on Summit Login Nodes as a User

We observe and analyze usage of the login nodes of the leadership class Summit supercomputer from the perspective of an ordinary user -- not a system administrator -- by periodically sampling user activities (job queues, running processes, etc.) for two full years (2020-2021). Our findings unveil key usage patterns that evidence misuse of the system, including gaming the policies, impairing I/O performance, and using login nodes as a sole computing resource. Our analysis highlights observed patterns for the execution of complex computations (workflows), which are key for processing large-scale applications.

==> sec-preprocessing.tex <==
\section{Data Preprocessing}

For the ease of processing, the raw data is programmatically converted to a consumable format. Following key information is organized into a comma separated values (csv) that stores the following information for each hour:

\begin{enumerate}
\item \texttt{login\_node} showing the login node information (login1-login5)
\item Number of logged in \texttt{users}
\item Number of \texttt{unique\_ips} the connection is being made from
\item Total number of user processed (\texttt{user\_procs})
\item CPU utilization in percent (\texttt{cpu\_util\_percent})
\item Memory utilization in percent (\texttt{memory\_util\_percent})
\item Disk utilization in percent (\texttt{disk\_util\_percent})
\item Time it takes to run an unaliased ls (\texttt{time\_to\_basic\_ls})
\item Time it takes to run a colored ls (\texttt{time\_to\_colored\_ls})
\item Time it takes to write 1G of random data to the scratch filesystem (\texttt{time\_to\_write\_1g})
\end{enumerate}




==> sec-results.tex <==
\section{Results}
\begin{enumerate}
\item An overall instantaneous state (need a catchy name) that defines the wholistic view of system - users logged in, cpu load, memory load -- identify most and least busy times based upon these
\item Load balance among the login nodes - state of the login nodes hourly over a typical month
\item User journey: Randomly pick 200 users and plot their journey: ``thinking time"
\item Type of applications being run on Login nodes -- classify by science area, programming language, CPU vs GPU
\item Evolution of storage space occupation -- how storage space gets taken up by evolving data
\item Identify potential misuse / abuse of resources based on the commands issued for processes
\item Scheduler and job stats: Avg. job size, walltime, total running / pending / suspended jobs at a time
\end{enumerate}

